Speed Scaling with Tandem Servers

Speed scaling for a tandem server setting is considered, where there is a series of servers, and each job has to be processed by each of the servers in sequence. Servers have a variable speed, their power consumption being a convex increasing function of the speed. We consider the worst case setting as well as the stochastic setting. In the worst case setting, the jobs are assumed to be of unit size with arbitrary (possibly adversarially determined) arrival instants. For this problem, we devise an online speed scaling algorithm that is constant competitive with respect to the optimal offline algorithm that has non-causal information. The proposed algorithm, at all times, uses the same speed on all active servers, such that the total power consumption equals the number of outstanding jobs. In the stochastic setting, we consider a more general tandem network, with a parallel bank of servers at each stage. In this setting, we show that random routing with a simple gated static speed selection is constant competitive. In both cases, the competitive ratio depends only on the power functions, and is independent of the workload and the number of servers.

==> SeriesParallel.tex <==
\section{Series of Parallel Servers}
In this section, we consider an even more general system model where there is series of parallel servers to closely model a network of servers. See Fig. 1 for an illustration, where there are layers of servers, with $M_k$ servers in layer $k$. Each layer $k$ has a single queue, where a job processed by any server of layer $k-1$ is stored before being processed on any server of layer $k$. New jobs arrive in the single queue of layer $1$ and are processed in serial order of layers.
The layered structure ensures that a job can be processed on any server in layer $\ell$ can only be processed only after it has been processed by some server in layer $\ell-1$.

To keep the analysis succinct, we consider just a two-layer setup, where layer $1$ has a single server, called {\it main}, followed by layer $2$ that has a parallel bank of $M$ servers. Extension to $K >2$ layers model follows similar to Section \ref{sec:hom}. 
We consider the homogenous setting where each job has same size on all the servers. 

%The heterogenous case can be solved identical to Section \ref{sec:het}, where the $k^{th}$  copy of newly arrived job $j$ with size $w_j^k$ is added to the queue of layer $k$ and the precedence constraint is enforced.

%In the homogenous/heterogenous setting, with identical job sizes on each server, the first claim (Proposition \ref{prop:rr_centralQ}) which helps the analysis is that $\opt$ assigns jobs processed by the main server to the $m$ parallel servers following a round-robin schedule. This claim also extends to any successive pair of layers, and makes the extension to multiple layer problem straightforward, since in each layer, jobs are assigned to different servers in a round robin fashion.

\begin{figure}\label{fig}
\begin{tikzpicture}[scale=0.850]
%\tikzstyle{};
%\foreach \x [count = \xi] in {2,3,4,5}
%{\node [rahulstyle] at (5,1+\xi) {};}
%\foreach \x [count = \xi] in {-1,0,...,4}
%{\node [rahulstyle] at (8,\xi) {};}
%\foreach \x [count = \xi] in {1,...,4}
%{\node [rahulstyle] at (12,1+\xi) {};}
%\foreach \x [count = \xi] in {-1, 0,...,4}
%{\node [rahulstyle] at (15,\xi) {};}
\draw[rounded corners] (4.65,1.5) rectangle (5.35,5.5);
\draw[rounded corners] (7.65,.5) rectangle (8.35,6.5);
%\draw[rounded corners] (11.5,.5) rectangle (12.5,6.5);
\draw[rounded corners] (6,3.25) rectangle (7,3.75);
%\draw[rounded corners] (9,3.25) rectangle (9,3.75);
\draw[rounded corners] (10,3.25) rectangle (11,3.75);

\draw[rounded corners] (11.65,1.5) rectangle (12.35,5.5);

%\draw[rounded corners] (14.5,.5) rectangle (15.5,6.5);
%\draw [->] (4.25,5.5) -- (4.25,1.5);
%\draw [->] (8.75,5.5) -- (8.75,1.5);
%\draw [->] (11.25,5.5) -- (11.25,1.5);
%\draw [->] (15.75,5.5) -- (15.75,1.5);

%\draw (5,6) -- (8,4);
%\draw (5,5) -- (8,6);
%\draw (5,3) -- (8,3);
%\draw (5,2) -- (8,1);
%\draw (5,4) -- (8,5);

%\draw (5,4) -- (8,5);
%\node [right,text width=2cm] at (8.1,5) {$x$};
\node [right,text width=2cm] at (8.3,6) {$1$};
\node [right,text width=2cm] at (8.3,1) {$M_2$};

%\node [left,text width=2cm] at (6.62,4) {$u'$};
\node [left,text width=2cm] at (6.5,5) {$1$};

\node [left,text width=2cm] at (6.5,2) {$M_1$};
%\node [right,text width=2cm] at (15.1,3) {$v'$};
%\node [right,text width=2cm] at (15.1,5) {$x$};
\node [right,text width=2cm] at (6.2,3.5) {$Q$};
%\node [right,text width=2cm] at (8.2,3.5) {$Q$};
\node [right,text width=2cm] at (10.2,3.5) {$Q$};


%\node [left,text width=2cm] at (4.75,3.5) {order of arrival};
%\node [left,text width=2cm] at (11,3.5) {increasing rank};
\node [left,text width=2cm] at (15,5) {$1$};
\node [left,text width=2cm] at (15,2) {$M_K$};

%\coordinate (A) at (5,5);
%\coordinate (B) at (6,5);
%\coordinate (C) at (7,3);
%\arcThroughThreePoints{A}{B}{C};

\coordinate [label=left:$$] (A) at (5,5);
\coordinate [label=left:$$] (B) at (5.5,4);
\coordinate [label=left:$$] (C) at (5.9,3.65);

\draw[thin, blue, ->] plot [smooth] coordinates { (A) (B) (C) };

\coordinate [label=left:$$] (A1) at (5,2);
\coordinate [label=left:$$] (B1) at (5.5,3);
\coordinate [label=left:$$] (C1) at (5.9,3.35);

\draw[thin,blue, -> ] plot [smooth] coordinates { (A1) (B1) (C1) };


\coordinate [label=left:$$] (A2) at (7,3.5);
\coordinate [label=left:$$] (B2) at (7.5,4.75);
\coordinate [label=left:$$] (C2) at (8,5);

\draw[thin,blue,->] plot [smooth] coordinates { (A2) (B2) (C2) };

\filldraw (9,3.5) circle (2pt);
\filldraw (9.25,3.5) circle (2pt);
\filldraw (9.5,3.5) circle (2pt);


%\coordinate [label=left:$$] (A3) at (8.3,2);
%\coordinate [label=left:$$] (B3) at (5.5,3);
%\coordinate [label=left:$$] (C3) at (6,3.5);
%
%\draw[thin,blue] plot [smooth] coordinates { (A3) (B3) (C3) };

%\draw (12,6) -- (15,4);
%\draw (12,5) -- (15,6);
%\draw[dashed] (12,4) -- (15,5);
%\draw (12,4) -- (15,3);
%\draw[dashed] (12,3) -- (15,3);
%
%\draw (12,2) -- (15,1);
%
%\draw (5,2) -- (8,1);
%\draw (12,3) -- (15,4);
\tikzset{rstyle/.style={draw,circle,scale = 0.3}}
%\node[rstyle=label text] (nodename) {};
\foreach \x [count = \xi] in {2,3,4,5}
{\node [rstyle] at (5,1+\xi) {};}
\foreach \x [count = \xi] in {-1,0,...,4}
{\node [rstyle] at (8,\xi) {};}
\foreach \x [count = \xi] in {1,...,4}
{\node [rstyle] at (12,1+\xi) {};}

\end{tikzpicture}
\caption{Series of layers of parallel servers with $M_k$ servers in layer $k$, with a common queue $Q$ for all server in each layer.}
\end{figure}


Let $n^{ij}(t)$ and $n_o^{ij}(t)$ the number of outstanding jobs on server $j$ of layer $i$ with the algorithm and the $\opt$, respectively at time $t$.
At time $t$, let $n^{ij}_o(t,q)$ and $n^{ij}(t,q)$
be the number of unfinished jobs with $\opt$ and the algorithm
respectively, on server $j$ of layer $i$ with remaining size at
least~$q$. Thus, $n^{ij}(t) = n^{ij}(t, 0)$ and $n^{ij}_o(t) = n^{ij}_0(t, 0)$.

The proposed algorithm assigns the job to multiple servers in layer $2$ as follows. We isolate one server from layer $2$, without loss of generality, let that be server $1$ of layer $2$. On each job departure from the main (only) server of layer $1$, the job is assigned to servers $2$ to $M$ of layer $2$ in a round-robin fashion as long they are idling. If all the servers $2$ to $M$ of layer $2$ are busy, then the departing job from the main server is assigned to the server $1$ of layer $2$. 
With this assignment policy, a natural way to define a potential function for each server is as follows. 

For the algorithm, server $i,1$ for $i=1,2$ is defined to be {\it active} if it has an unfinished job $n^{i1}(t) > 0$, and denote it by $A_i(t)=1$ if server is active and $A_i(t)=0$, otherwise. Then 
$A(t) = \sum_{i=1}^K A_i(t)$ is the number of active servers among the two first servers of the two layers with the algorithm.

For the main server in layer $1$, let $d^{11}(t,q) = \max\left\{0, n^{11}(t,q) - n^{11}_o(t,q)\right\}$, while for server $1$ of layer $2$  
%Let $q_{min}$ be a universal lower bound on the size of any job.
 $d^{21}(t,q)= \max\left\{0, \sum_{k=1}^{i-1} \left((n^{11}(t) - n^{11}_o(t)) + \max\left\{n^{21}(t,q) - n^{21}_o(t,q), 0\right\}\right) \right\}$.
 and server $j\ge 2$ of layer $2$,
 $d^{2j}(t,q) = \max\left\{0, n^{2j}(t,q) - n^{2j}_o(t,q)\right\}$.
For $i=1,2$, let 
$\Phi_{i1}(t) =   c_{i1} \int_{0}^1 f\left(\frac{d^{ij}(t,q)}{A(t)}\right) dq$, and 
for $i=2, j \ge 2$
$\Phi_{ij}(t) =   c_{ij} \int_{0}^1 f\left(d^{ij}(t,q)\right) dq$.
Then consider the potential function \begin{equation}\label{defn:phiSP}
\Phi(t)=\sum_{i,j}\Phi_{ij}(t),
\end{equation} 
where $f(0) = 0$, and $\forall \ i\ge 1$, $ f\left(\frac{i}{A(t)}\right)-f\left(\frac{i-1}{A(t)}\right) = \Delta\left(\frac{i}{A(t)}\right) :=
P'\left(P^{-1}\left(\frac{i}{A(t)}\right)\right)$ (this means $P'(x)$ where $x=P^{-1}\left(\frac{i}{A(t)}\right)$). 
 
 {\bf Algorithm: } The speed scaling algorithm that we propose, chooses
the following speeds for servers. 
For server $1,1$, $s_{11}(t) = P^{-1}\left(\frac{n^{11}(t)+A(t)}  {A(t)}\right)$,  and for server $2,1$ whenever it is active, i.e.,  $A_2=1$, 
\begin{equation}\label{eq:speeddefSP}
 s_{21}(t) = \begin{cases}   P^{-1}\left(\frac{n^{11}(t)+A(t)}  {A(t)}\right), & \text{if} \ n^{11}(t)> 0, \\
 P^{-1}(2), &\text{otherwise.}\end{cases}
 \end{equation}
 For servers $2,j$, $j = [2 \dots m]$, 
 \begin{equation}\label{eq:speeddeflayer2}
s_{2j}(t) =  \begin{cases} P^{-1}(2), & \text{if} \ n^{2j}(t)> 0, \\
 0, &\text{otherwise.}\end{cases}
 \end{equation}
% Similar to Section \ref{sec:hom}, we need the following adjustment to job sizes only for the algorithm in a certain case.
% \begin{remark}\label{rem:jumpSP}
% If $n^{11}(t)= 0$, and a new job arrives at server $1$ at time $t^+$, let the size of the outstanding job on active server 
%$2,1$ at time $t$ be $q_{21}\le 1$. For ease of analysis,  
%we increase the size of the existing job on active servers $2,1$ to $q_{21}=1$ at time $t^+$ only for the algorithm. If $q_{21}=0$, then no increase is needed. This only increases the work/cost  for the algorithm and not the $\opt$.
% \end{remark}
% 
Essentially, the assignment policy and the speed scaling algorithm creates a tandem system of one server each in both the layers, and makes the other servers of layer $2$ work independently (at speed of $P^{-1}(2)$) of the number of jobs available at server $1$.
For a general system with multiple servers in each layer, and let the minimum number of servers across layers be $M_{\min}$. Then the algorithm will isolate $M_{\min}$ servers from each layer and operate a tandem system of $M_{\min}$ parallel servers in each layer, and use the other servers in each layer to work independently (at speed of $P^{-1}(2)$) of the total number of jobs in the system. Therefore results presented in this section can be extended to a general system in a straightforward manner following Section \ref{sec:hom}.

 
\begin{lemma}\label{lem:jumpSP}
The total increase in $\Phi(t)$ at discontinuous points is at most $4 c n  f(1)$.
\end{lemma}


 \begin{lemma}\label{lem:driftSP}
When $n^{11}(t)>0$, for any active server $i,1$ for $i=1,2$ 
\begin{align*}d\Phi_{i1}/dt\le  c_{i1} P(s_{i1}^o) - c_{i1} \frac{n^{11}(t) + i-1}{A(t)} + c_{i1} \frac{n^{11}_o(t) + \sum_{i=1}^{2}\b1^{i1}_o(t) n^{i1}_o(t)}{A(t)}  
\end{align*}
where $\b1^{ij}_o(t)=1$ if server $ij$ is active with the $\opt$ and $0$ otherwise,
and $d\Phi_{i1}/dt = 0$ for any inactive server. 
When $n^{11}(t)=0$, for active server $2,1$
$$d\Phi_{21}(t)/dt  = c_{21}\left(P(s_{21}^o) - c_{21}  + c_{21} \frac{n^{11}_o(t) + \b1^{21}_o(t) n^{21}_o(t)}{A(t)} \right)$$ and $d\Phi_{i1}/dt = 0$ for any inactive server among $1,1$ and $2,1$.
Moreover, when server $2,j$ is active, then
$$d\Phi_{2j}/dt\le c_{2j} P(s_{2j}^o) - c_{2j} n^{2j}(t) + c_{2j}n^{2j}_o(t),$$
and $d\Phi_{2j}/dt=0$, otherwise.
\end{lemma}

\begin{theorem}\label{thm:mainSP}
  The proposed speed scaling algorithm \eqref{eq:speeddefSP} is
  $c$-competitive with the two-layer series parallel servers with homogenous jobs,
  where $$c = 6(1+ f(1)).$$
\end{theorem}
Proof of Theorem \ref{thm:mainSP} is identical to Theorem \ref{thm:main} using Lemma \ref{lem:jumpSP} and \ref{lem:driftSP}.


